One-Hop Sub-Query Result Caches for Graph Database Systems

This paper introduces a novel one-hop sub-query result cache for processing graph read transactions, gR-Txs, in a graph database system. The one-hop navigation is from a vertex using either its in-coming or out-going edges with selection predicates that filter edges and vertices. Its cache entry identifies a unique one-hop sub-query (key) and its result set consisting of immutable vertex ids (value). When processing a gR-Tx, the query processor identifies its sequence of individual one-hop sub-queries and looks up their results in the cache. A cache hit fetches less data from the storage manager and eliminates the requirement to process the one-hop sub-query. A cache miss populates the cache asynchronously and in a transactional manner, maintaining the separation of read and write paths of our transactional storage manager. A graph read and write transaction, gRW-Tx, identifies the impacted cache entries and either deletes or updates them. Our implementation of the cache is inside the graph query processing engine and transparent to a user application. We evaluate the cache using our eCommerce production workload and with rules that re-write graph queries to maximize the performance enhancements observed with the cache. Obtained results show the cache enhances 95th and 99th percentile of query response times by at least 2x and 1.63x, respectively. When combined with query re-writing, the enhancements are at least 2.33x and 4.48x, respectively. An interesting result is the significant performance enhancement observed by the indirect beneficiaries of the cache, gRW-Txs and gR-Txs that do not reference one-hop sub-queries. The cache frees system resources to expedite their processing significantly.

==> FDButil.tex <==
\begin{figure*}[htbp]  % htbp defines position as here, top, bottom, page



    % Group 2 (Middle: 3 Charts)
    \begin{subfigure}{\linewidth}
        \centering
        \begin{subfigure}{0.32\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/FDB Storage CPU.pdf}
        \end{subfigure}
        % \hspace{0.03\linewidth}
        \begin{subfigure}{0.32\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/FDB Storage Disk Busy.pdf}
        \end{subfigure}
        % \hspace{0.03\linewidth}
        \begin{subfigure}{0.32\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/FDB Storage Network Sent.pdf}
        \end{subfigure}
        \caption{FDB storage nodes}
        \label{fig:fdb_storage_utilization}
    \end{subfigure}

    \vspace{1em}  % Space between groups

    % Group 3 (Bottom: 3 Charts)
    \begin{subfigure}{\linewidth}
        \centering
        \begin{subfigure}{0.32\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/FDB Transaction CPU.pdf}
        \end{subfigure}
        % \hspace{0.03\linewidth}
        \begin{subfigure}{0.32\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/FDB Transaction Disk Busy.pdf}
        \end{subfigure}
        % \hspace{0.03\linewidth}
        \begin{subfigure}{0.32\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/FDB Transaction Network Sent.pdf}
        \end{subfigure}
        \caption{FDB transaction nodes}
        \label{fig:fdb_xact_utilization}
    \end{subfigure}

    \caption{CPU, Disk, and Network utilization of FDB storage and transaction nodes with $\widehat R$.}
    \label{fig:fdb_read_utilization}
\end{figure*}

\begin{figure*}[htbp]  % htbp defines position as here, top, bottom, page
    % Group 3 (Bottom: 3 Charts)
    \begin{subfigure}{\linewidth}
        \centering
        \begin{subfigure}{0.32\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/[Write] FDB Transaction CPU.pdf}
        \end{subfigure}
        % \hspace{0.03\linewidth}
        \begin{subfigure}{0.32\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/[Write] FDB Transaction Disk Busy.pdf}
        \end{subfigure}
        % \hspace{0.03\linewidth}
        \begin{subfigure}{0.32\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/[Write] FDB Transaction Network Sent.pdf}
        \end{subfigure}
        % \caption{FDB transaction nodes}
        \label{fig:fdb_xact_utilization}
    \end{subfigure}

    \caption{CPU, Disk, and Network utilization of FDB transaction nodes with $\widehat W$.}
    \label{fig:fdb_write_utilization}
\end{figure*}

==> discuss.tex <==
A workload may references a certain property value of an edge or vertex with a high frequency.
For example, our workload uses \texttt{“Status”=0} with a high frequency while other \texttt{“Status”} values are rarely referenced.
Caching the result of one-hop sub-query instances with rare values provides little to no performance benefit.
%This is for the obvious reason that they are accessed rarely.
They may degrade the performance of gRW-Txs by requiring them to either invalidate or refill potentially non-existent caches entries.
Non-existent because the cache entry has either been evicted by the cache replacement policy due to their low recency of references or was invalidated by a previous write.

We address this by allowing a one-hop sub-query template to specify a frequently accessed value in its predicate (instead of a wildcard).
It is a hint to the query processor to cache the result of sub-queries with the specified value for the property.
And, it prevents writes from invalidating/refilling cache entries that do not use the frequently accessed value.
To illustrate, consider the following query template: {\small\texttt{\_\_.outE(‘Linking’).has(“IsActive”, *).inV().has(“Status”, 0)}}.
It causes the query processor to cache the result of one-hop sub-query instances with \texttt{“Status”=0} for leaf vertices.
Thus, a one-hop sub-query instance with \texttt{“Status”=1} will not be cached.
Moreover, a gRW-Tx invalidates/refills only those cache entries corresponding to one-hop sub-query instances with \texttt{“Status”=0}.
Note that with \texttt{“Status”='?'}, every time the value of \texttt{“IsActive”} is updated with a root vertex $V_i$ that has a high fan-out, a large number of redundant invalidations/refills may have to be performed on a rarely referenced \texttt{“Status”} value.
This is especially true when the different \texttt{“Status”} values have the same probability of occurrence.
This is prevented by replacing the wildcard with the frequently referenced value.

% A gRW-Tx processes different one-hop sub-queries that may require the vertex properties.
% Our implementation requires the gRW-Tx to identify the properties referenced by the different one-hop sub-queries at its initialization time.
% The gRW-Tx obtains the value of these properties once and uses them to compute the impacted cache entries.

%It is possible to have a sub-query template with a value for a property.  This enhances the performance of writes when a small percentage of queries use a \texttt{“Status”} property value different than zero by eliminating the unnecessary invalidation/refill attempts on non-existent cache keys.  Limit to a constant value reduces the unnecessary update overhead on non-exist cache keys with different Status values if there is never/very little queries that query on different Status values. Assume an ip_address  connects with 10 accounts where 4 of them have Status=0 and 6 of them have Status=1. Then the result of the cache template in the previous email on this ip address is 4 vertex ids (assume IsActive=true on all edges). Updating an edge property on one of the edges connecting to the other 6 accounts does not impact the result, so the cache entry does not need to be invalidated.



==> eval.tex <==


% Characterize the production workload and how it uses the cache:
% \begin{itemize}
% \item Read to write ratio.
% \item Number of sub-query templates and how they are shared across the different query templates.
% \item Number of sub-query instances for each query template.
% \item Number of sub-query instances shared across different query templates.

% \item Frequency of the 9 different writes.  
% \item The different writes and their frequency.
% \item The number of sub-query templates invalidated by a write.
% \end{itemize}

% \noindent We require scientific numbers showing the benefits of the cache:
% \begin{itemize}
% \item Performance enhancements observed by re-writing queries.
% \item Performance enhancements observed by using the cache with the original and re-written queries.
% \end{itemize}

% \noindent And, scientific numbers showing the overhead of the cache:
% \begin{itemize}
% \item Performance of writes with and without the cache.  What is the impact on their latency? 
% \end{itemize}

\begin{figure}
  \begin{center}
    \includegraphics[width=0.9\columnwidth]{figs/mirroring_v2.pdf}%mirroring.png}
  \end{center}
  \caption{Evaluation using mirrored traffic from a production system.}\label{fig:mirrored}
\end{figure}

%{\color{blue}

%Existing benchmarks do not resemble well our production workload and may produce inadequate results for our solution.
%Instead of evaluating on existing benchmarks, 

Our FoundationDB deployment is across three data centers using its asymmetric configuration model~\cite{fdb7,fdbconfig} for high availability. %\footnote{\href{https://apple.github.io/foundationdb/configuration.html#asymmetric-configurations}{https://apple.github.io/foundationdb/configuration.html#asymmetric-configurations}}. 
Two data centers, primary and secondary, have a replica of the graph database.
Each constructs three copies of data. 
The third data center hosts the transaction log records only.

We mirrored the traffic from our Production system to a Test system to quantify the tradeoffs associated with our one-hop sub-query result cache.
%We mirrored graph queries and writes traffic from our production system to a testing system to evaluate the performance of our caching solution, see Figure~\ref{fig:mirrored}.
Both systems have the same hardware.
Each consists of 288 FDB nodes.
The Test system consists of 180 Graph-QP nodes deployed in the primary data center.
%We evaluated the traffic with cache in the primary data center where 180 Graph-QP nodes are deployed. 
%The data size is 7.8TB (61.4TB on disk). 
Each FDB node consists of 3 cores and 18 GB of memory.
It runs 2 FDB processes.
Each Graph-QP node consists of 3 cores and 16 GB of memory.
%This is done by setting up a testing FoundationDB cluster with the same size and similar hardware as the production FDB cluster.
%The most recent backup copy of the production data is restored on the testing FDB cluster.


We fork graph queries, inserts, updates, and deletes from the Production system by configuring its Graph-QP to place the graph operation
in a queue and process it normally.
To simplify discussion and without loss of generality, we refer to graph queries as reads and graph inserts, updates, and deletes as writes for the rest of this section.
%Requests issued to the production system are placed in a queue while being served normally.
%Production requests are put in queues, while still being served normally at the production deployment. 
In the background, these queued requests, including both reads and writes, are forwarded to the graph nodes of the Test system, see Figure~\ref{fig:mirrored}.
The data in the Production and Test systems are almost identical. 
We are not comparing the Production system with the Test system. 
We are comparing the Test system with itself by adjusting its configuration, e.g., turn the cache on and off to see the impact on the 95$^{th}$ and 99$^{th}$ latency.
%The Production system forks its requests to the Test system for the experimental results presented in this section.
%evaluation purposes. 



%The data in the Production and Test systems are not identical, but is sufficient enough for us to reproduce the similar request rate (requests/sec) and overall latency, thus sufficient to evaluate our caching solution.

%Both the production and testing deployments each consists of 288 FDB nodes in a 3-datacenter setup, along with 180 service nodes. The data size is 7.8TB (61.4TB on disk). Each FDB node is 3-core, 18GB-memory and has 2 FDB processes running.
%Each graph node is 3-core, 16GB-memory runs our graph service that employs the modified JanusGraph software to be cache-aware.

\input{queryRewriting}

\subsection{Production Traffic Pattern}

Fig~\ref{fig:traffic_pattern} shows four days of our production workload in the primary datacenter, highlighting its diurnal characteristics.
It consists of three distinct loads:
\begin{enumerate}
    \item $\widehat R$: A high system load of approximately 2k-3k graph queries/second from 11 am to 1 pm.
    \item $\widehat W$: The heaviest graph write load from 3-5 pm daily during an offline batch write process that starts at 3 pm and may last for approximately 4-12 hours.
    \item $\widecheck R$: A low system load of approximately 1k graph queries/second from 9-11 pm.    
\end{enumerate}
Both read dominated workloads, $\widehat R$ and $\widecheck R$, include approximately 30 graph write requests per second. 
%A similar production traffic pattern is repeated each day. Fig~\ref{fig:traffic_pattern} shows the traffic of our 4-day traffic pattern. Each day the peak read traffic ranges from 2-2.5k requests/sec around 11am-1pm, while the low read traffic is around 1k requests/sec that happens at 9-11pm. Small online write traffic of around 30 requests/sec happens during the day, while there are some offline-batch-write traffic starts from 3pm and ends around 3am with a long tail (heaviest write traffic is normally at 3-5pm). Therefore, we define three periods of the workload that are of interests: low read traffic ($\widecheck R$), peak read traffic ($\widehat R$), and heavy write traffic ($\widehat W$).
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/traffic_pattern.pdf}
    \caption{Production traffic pattern for 4 days}
    \label{fig:traffic_pattern}
\end{figure}
%In this workload, online write traffic These writes are batches that 
Each inserts or updates a small number of vertices and edges. 
%Due to external data pipeline relying on other sources, some data might be missed. 

With $\widehat W$, each write consists of a larger batch described in Section~\ref{sec:write_fine}.
%that serves two purposes: (1) update vertices and edges, and (2) delete old edges based on their timestamp properties to make GraphQP's processing of queries more efficient.
Although write traffic based on request count during write-heavy period is as high as 34\%, the actual number of changes (as listed in Section~\ref{sec:writes}) is not that high. As we show later in Section~\ref{sec:write_analysis}, the overhead of writes to detect and invalidate cache entries is negligible. 
%Moreover, since a large percentage of graph writes checks for conditions that are not satisfied, write latency is even reduced due to lower read loads due to caching imposed on both the database and the graph query processors.
A large percentage of our graph writes are read-modify-writes (RMW) that check for a condition after reading the data.
After the read, should the condition not be satisfied, no modification or write is performed. 
With our application, the conditions are not satisfied most of the time.
While a read of RMW may reference a one-hop sub-query template, we do not service it using the cache.
This ensures reads of a complex RMW observes its own partial writes.
%Write latency improves due to lower read loads due to caching imposed on both the database and the graph query processors. 


We enabled query logs on the Test system to collect query statistics, including query templates, traffic distributions, and latency metrics.
Our workload consists of approximately 150 unique query templates.
We excluded the query templates that contributed less than 1\% traffic.
With the remaining query templates, six one-hop sub-query templates are identified for caching\footnote{It is interesting to note that some of the 1\% queries that were not considered do reference one or more of these one-hop sub-query templates.}.
%For the remaining query templates, we identified six sub-query templates for caching that were used in our evaluation.  
These cover \textasciitilde36\% of query templates, which account for more than \textasciitilde68\% of the graph queries issued to the Test system. We enabled caching these sub-query templates for two weeks until reads reached a reasonably high cache hit rate (86\% for the combined six sub-query templates). Table~\ref{tbl:sub_query_templates} summarizes the six sub-query templates and their range of cache hit rates at the time the experiments were conducted. SQ1 and SQ2 traverse the outgoing edges of root vertices, while SQ3-6 traverse the incoming edges of root vertices. 


\begin{table}[!ht]
    \centering
    \begin{tabular}{|l|l|l|}
        \hline
        Name & Cache Hit Rate \\ \hline
        SQ1 & 82-86\% \\ \hline
        SQ2 & 80-86\% \\ \hline
        SQ3 & 82-88\% \\ \hline
        SQ4 & 84-89\%\\ \hline
        SQ5 & 90-93\%\\ \hline
        SQ6 & 86-90\%\\ \hline
    \end{tabular}
    \caption{Six sub-query templates used in our evaluation}
    \label{tbl:sub_query_templates}
\end{table}

% \begin{table}[!ht]
%     \centering
%     \begin{tabular}{|c|cc|cc|cc|}
%     \hline
%     \multirow{2}{*}{Period}    & \multicolumn{2}{c|}{August 25} & \multicolumn{2}{c|}{August 26} & \multicolumn{2}{c|}{August 27} \\
%     \cline{2-7}
%         & Original & Rewrite & Original & Rewrite & Original & Rewrite \\
%     \hline
%          $\widecheck R$& 1.72 & 1.72 & 1.70 & 1.68 & 1.74 & 1.82 \\ \hline
%          $\widehat R$& 1.68 & 1.77 & 1.50 & 1.48 & 1.44 & 1.52 \\ \hline
%          $\widehat W$& 1.59 & 1.54 & 1.50 & 1.59 & 1.47 & 1.73\\ \hline
%     \end{tabular}
%     \caption{Factor of improvement observed by indirect beneficiaries of the cache, 14.2\% of workload, cache enabled, 99$^{th}$\%.}
%     \label{tbl:restofqueries99}
% \end{table}

\begin{table*}[!ht]
    \centering
    \begin{tabular}{|c|c|c|c||c|c|c||c|c|c|}
        \hline
        \multirow{2}{*}{Query} & \multirow{2}{*}{\% Traffic} & \multirow{2}{*}{Re-writable?} & Referenced One-Hop  & \multicolumn{3}{|c||}{\textbf{95$^{th}$ Percentile Read}} & \multicolumn{3}{|c|}{\textbf{99$^{th}$ Percentile Read}} \\ \cline{5-10}        
        & & & Sub-Query Templates & C$^-$Q$^+$ & C$^+$Q$^-$ & C$^+$Q$^+$ & C$^-$Q$^+$ & C$^+$Q$^-$ & C$^+$Q$^+$ \\ \hline \hline
Q1  & 14.55\% & \no & -- & 1.00 & 6.11  & 6.11  & 0.99 & 1.74 & 1.83  \\
Q2  & 4.88\%  & \yes  & SQ2, SQ5                      & 1.04 & 6.06  & 10.78 & 1.04 & 2.01 & 2.13  \\
Q3  & 4.83\%  & \no & -- & 1.01 & 12.71 & 12.71 & 1.01 & 1.76 & 1.74  \\
Q4  & 4.78\%  & \yes  &  SQ2, SQ3                     & 0.99 & 10.44 & 10.44 & 0.96 & 2.03 & 2.07  \\
Q5  & 4.77\%  & \yes  & SQ2 (2), SQ5 (2)                       & 0.97 & 4.71  & 3.23  & 0.94 & 2.63 & 2.45  \\
Q6  & 4.76\%  & \yes  & SQ2, SQ5                       & 4.07 & 1.17  & 33.58 & 7.02 & 1.37 & 15.10 \\
Q7  & 4.70\%  & \yes  & SQ2, SQ5                      & 1.02 & 6.33  & 10.56 & 0.99 & 1.91 & 2.01  \\
Q8  & 4.07\%  & \no & -- & 1.00 & 8.67  & 8.67  & 1.00 & 1.66 & 1.66  \\
Q9  & 3.45\%  & \yes  & SQ2 (2), SQ5 (2)                      & 1.03 & 4.69  & 3.70  & 1.09 & 5.76 & 4.60  \\
Q10 & 3.40\%  & \yes  & SQ2 (2), SQ5 (2)                      & 1.25 & 2.27  & 3.80  & 1.52 & 1.25 & 4.04  \\
Q11 & 3.33\%  & \yes  & SQ2, SQ3                      & 1.02 & 2.93  & 12.30 & 0.98 & 2.40 & 2.97  \\
Q12 & 3.03\%  & \yes  & SQ1, SQ4                       & 1.05 & 0.74  & 21.20 & 1.01 & 1.48 & 37.63 \\
Q13 & 2.93\%  & \yes  & SQ1, SQ6                      & 2.10 & 1.05  & 5.59  & 0.79 & 1.04 & 2.07  \\
Q14 & 2.17\%  & \yes  & SQ1, SQ4                      & 1.01 & 5.20  & 5.47  & 0.99 & 2.13 & 2.20  \\
Q15 & 2.09\%  & \yes  & SQ1, SQ6                      & 1.01 & 5.15  & 5.42  & 1.05 & 2.13 & 2.23  \\
Q16 & 2.09\%  & \yes  & SQ1, SQ4                      & 1.01 & 6.31  & 5.94  & 0.97 & 2.04 & 2.04  \\
Q17 & 2.03\%  & \yes  & SQ1, SQ6                      & 0.99 & 6.31  & 6.31  & 0.98 & 2.06 & 2.11  \\
Q18 & 1.85\%  & \no & SQ1 & 1.01 & 9.18  & 9.18  & 0.99 & 2.08 & 2.10  \\
Q19 & 1.81\%  & \yes  & SQ2, SQ3                      & 1.02 & 9.60  & 9.60  & 1.02 & 1.99 & 2.05  \\
Q20 & 1.80\%  & \yes  & SQ2 (2), SQ5 (2)                      & 1.01 & 9.09  & 7.69  & 0.97 & 2.10 & 2.10  \\
Q21 & 1.80\%  & \yes  & SQ2 (2), SQ5 (2)                      & 1.01 & 7.31  & 7.92  & 0.95 & 1.91 & 1.91  \\
Q22 & 1.80\%  & \yes  & SQ1, SQ2, SQ5                      & 0.99 & 4.83  & 5.05  & 0.98 & 2.35 & 2.37  \\
Q23 & 1.80\%  & \yes  & SQ2 (2), SQ5 (2)                      & 1.01 & 6.50  & 6.12  & 0.97 & 2.26 & 2.24  \\
Q24 & 1.80\%  & \yes  & SQ2 (2), SQ5 (2)                      & 1.00 & 7.36  & 6.87  & 0.97 & 2.33 & 2.30  \\
Q25 & 1.74\%  & \yes  & SQ4                      & 0.99 & 3.47  & 3.71  & 0.95 & 1.89 & 1.96  \\
Q26 & 1.72\%  & \yes  & SQ2 (2), SQ5 (2)                      & 1.07 & 2.76  & 2.81  & 1.33 & 4.10 & 4.57  \\
Q27 & 1.37\%  & \no  & SQ6 & 1.05 & 2.91  & 3.37  & 1.03 & 1.92 & 2.00 \\
\hline         
%\hline
    \end{tabular}
    \caption{Factor of improvement in latency with $\widehat R$ using either query-rewriting, cache, or both. The number in parenthesis, see Column 4, shows how many times a sub-query template is referenced by a query.}
    \label{tbl:query_template_latency}
\end{table*}


%With each workload listed in Table~\ref{tbl:workload_periods}, we ran four configurations below, each for 30 minutes where 5 minutes were accounted for configuration switching:
With the Test system, we may enable or disable the cache. 
These are denoted as C$^+$ and C$^-$, respectively.
Similarly, we may enable or disable query re-writing, denoted Q$^+$ and Q$^-$, respectively.
Hence, the Test system supports four possible configurations:
\begin{enumerate}
  \item \textbf{C$^-$Q$^-$}: Disable cache and disable query re-writing.
  \item \textbf{C$^-$Q$^+$}: Disable cache and enable query re-writing.
  \item \textbf{C$^+$Q$^-$}: Enable cache and disable query re-writing.  
  \item \textbf{C$^+$Q$^+$}: Enable cache and enable query re-writing.
\end{enumerate}






\begin{figure}[!ht]
    \centering
    \includegraphics[width=\linewidth]{figs/occurrences.jpeg}
    \caption{Number of occurrences of 3 queries in 25-minutes during peak traffic on Day 1.}
    \label{fig:3q}
\end{figure}

\color{black}
\noindent{\em Uniform Occurrence of Query Instances:}
For a given workload and a 25-minute evaluation window, query instances occur with approximately a uniform distribution. 
Figure~\ref{fig:3q} highlights this by showing the occurrences of instances of three query templates during one 30 minute session.
We identify each query instance with a unique integer id.
We quantify the number of times a query instance occurs. 
The x-axis is the id and the y-axis is the number of times the query occurs.
Both axes are in log scale.
%The x-axis of this figure is log scale, identifying the different query instances by a unique identifier.  
%The y-axis, also in log scale, is the number of times a query instance is issued.
The line charts show different query templates identified using their hash.
We selected these query templates because they reference a different number of one-hop sub-query templates.
While 
Query template 4e918f85 references 4 one-hop sub-query templates, 9d5faa33 consists of 2 one-hop sub-query templates, and b5b2398d consists of 1 one-hop sub-query template.
With b5b2398d, one query instance out of 67,814 issued queries occurs 586 times.
The total number of query instances issued 3 or more times is less than 9\% of all b5b2398d query instances.
This percentage is lower with the other two query templates.
While the queries are unique, as shown in Table~\ref{tbl:sub_query_templates}, the cache hit rate for the sub-query results that constitute the graph queries is high.
This is because the cache has been in-use for approximately 2 weeks.


%In the following sub-sections, we will evaluate system reads, writes, error rates, and resource utilization across various workloads and configurations.
Below, we describe the overall performance of the system.
Subsequently, we describe the performance of reads and writes separately.



\subsection{Coarse-Grained Analysis}\label{sec:eval_coarse}
Table~\ref{tbl:workload_periods} shows the overall percentage of reads and writes that constitute the different workloads, and the overall 95$^{th}$ and 99$^{th}$ percentile latency of reads and writes.
These are without query re-writing and the one-hop sub-query result cache, C$^-$Q$^-$.
This table shows $\widecheck R$ observes the fastest read and write latency due to a low system load.
The cache, query re-writing, and their combination expedite both the 95$^{th}$ and 99$^{th}$ percentile latency significantly, see Figures~\ref{fig:overall_95_read_latency} and~\ref{fig:overall_99_read_latency}.
Both normalize the latency observed with C$^+$Q$^+$ and $\widecheck R$ as one and show the factor of slow-down with the other settings.
%(without cache) for each workload as our base line.
%Fig~\ref{fig:overall_95_read_latency} shows the 95$^{th}$ percentile read latency with different workloads and system configurations, normalized by the C$^+$Q$^+$ latency of the $\widecheck R$ as shown in Table~\ref{tbl:workload_periods}.
%(C$^+$Q$^+$ latency is shown as 1). 
Read latency is highest with $\widehat R$, followed by $\widehat W$, and is lowest during $\widecheck R$. The cache improves the latency by more than 2x for all workloads. The cache combined with query rewriting improves the latency by more than 3x.

\begin{table}[!ht]
    \centering
    \small
    \begin{tabular}{|c||c|c|cc|cc|}
    \hline
         \multirow{2}{*}{Workload}&  \multirow{2}{*}{\% Reads} &  \multirow{2}{*}{\% Writes} &  \multicolumn{2}{c|}{Read Latency (ms)}& \multicolumn{2}{c|}{Write Latency (ms)}\\ 
         \cline{4-7}
               &  &  & 95$^{th}$\% & 99$^{th}$\% & 95$^{th}$\% & 99$^{th}$\% \\
        \hline
        \hline
         $\widehat R$&  99\%&  1\%&  130 & 989 & 137 & 317 \\ \hline
         $\widehat W$&  62\%&  38\%&  96 & 773 & 105 & 197 \\ \hline
        $\widecheck R$&  94\%&  6\%&  73 & 693 & 91 & 171\\ \hline
    \end{tabular}
    \caption{C$^-$Q$^-$, different workloads and their latency.}
    \label{tbl:workload_periods}
\end{table}

% Based on Aug 27 data
\begin{table*}
    \centering
    \begin{tabular}{|c||ccc|ccc|}
    \hline
        \multirow{2}{*}{Workload} & \multicolumn{3}{c|}{95$^{th}$\% Latency} & \multicolumn{3}{c|}{99$^{th}$\% Latency} \\
        \cline{2-7}
         & C$^-$Q$^+$ & C$^+$Q$^-$ & C$^+$Q$^+$ & C$^-$Q$^+$ & C$^+$Q$^-$ & C$^+$Q$^+$ \\ \hline
        $\widehat R$ & 1.10 & 2.06 & 3.17 & 1.36 & 1.63 & 4.90 \\ \hline
        $\widehat W$ & 1.17 & 2.04 & 2.59 & 1.59 & 1.72 & 4.66 \\ \hline
        $\widecheck R$ & 1.16 & 2.31 & 3.70 & 1.33 & 1.87 & 5.21 \\
    \hline
    \end{tabular}
    \caption{Factor of improvement in the 95$^{th}$\% and 99$^{th}$\% latency of graph queries.}
    \label{tab:my_label}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{|c||ccc|ccc|}
    \hline
        \multirow{2}{*}{Workload} & \multicolumn{3}{c|}{95$^{th}$\% latency} & \multicolumn{3}{c|}{99$^{th}$\% latency} \\
        \cline{2-7}
         & C$^-$Q$^+$ & C$^+$Q$^-$ & C$^+$Q$^+$ & C$^-$Q$^+$ & C$^+$Q$^-$ & C$^+$Q$^+$ \\ \hline
        $\widehat R$ & 0.99 & 1.10 & 1.76 & 1.00 & 1.47 & 1.99 \\ \hline
        $\widehat W$ & 1.02 & 1.44 & 1.40 & 1.01 & 1.32 & 1.40 \\ \hline
        $\widecheck R$ & 1.01 & 0.98 & 0.98 & 0.98 & 1.25 & 1.24 \\
    \hline
    \end{tabular}
    \caption{Factor of improvement in the 95$^{th}$\% and 99$^{th}$\% latency of writes.}
    \label{tab:my_label}
\end{table*}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.8\linewidth]{figs/overall_95_read_latency_normalized.pdf}
    \caption{95$^{th}$ normalized read latency with different workloads.}
    \label{fig:overall_95_read_latency}
\end{figure}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.8\linewidth]{figs/overall_99_read_latency_normalized.pdf}
    \caption{99$^{th}$ normalized read latency with different workloads.}
    \label{fig:overall_99_read_latency}
\end{figure}


\input{graphQPutil}

Table~\ref{tbl:impactedKyes} shows the number of cached entries impacted by the writes.
The maximum number of impacted keys with the read dominated workloads, $\widecheck R$ and $\widehat R$, is in the order of tens and hundreds.

The cache reduces the overhead of query processing.
It frees resources to enhance the performance of writes and queries that are not able to use the cache.
(See Sections~\ref{sec:read_fine} and~\ref{sec:write_fine} for details.)
Figure~\ref{fig:graphQPutil} show the CPU utilization of a Graph-QP node with $\widehat R$.
It consists of a single threaded FDB client component that processes network I/O to the FDB cluster.
A lower network traffic reduces the CPU utilization of this thread.  
%Its CPU utilization is shown in Figure~\ref{fig:fdb-thread-util}. 
%It consists of one thread and processes network I/O to the FDB cluster.
Figure~\ref{fig:fdb-thread-util} shows
its CPU consumption is reduced dramatically with $C^{+}Q^{+}$, reducing the overall CPU utilization of the Graph-QP instance significantly, see Figure~\ref{fig:graph-qp-util}.

%to free resources for processing writes and queries that do not use the cache. 
%We discuss the write that invalidates 2516 keys in Section~\ref{sec:write_fine}

\begin{table}[!ht]
    \centering
    \begin{tabular}{|l||c|c|c|c|c|}
        \hline
         & Min & 50th & 95$^{th}$ & 99$^{th}$ & Max \\ \hline
 $\widehat R$ & 0 & 8 & 16 & 24 & 272 \\
 \hline
 $\widehat W$ & 0 & 0 & 16 & 22 & 2516 \\ \hline
 $\widecheck R$ & 0 & 0 & 16 & 32 & 52 \\ \hline
    \end{tabular}
    \caption{Number of invalidated cache entries per graph write.}
    \label{tbl:impactedKyes}
\end{table}

\input{FDButil}

Figure~\ref{fig:fdb_read_utilization} shows the utilization of the FDB storage and transaction nodes with $\widehat R$.
Figure~\ref{fig:fdb_storage_utilization} shows the cache reduces the load imposed on the FDB CPU, disk, and network by reducing their utilization.
The network utilization is reduced by almost 4x and the disk utilization is reduced by almost 2x. 
These results highlight sub-query cache lookups is more efficient than processing the sub-queries.

With the cache, the sub-queries that observe a cache miss cause the 
background CP threads to compute cache entries and insert them in FDB in a transactional manner.
They use FDB's transaction nodes such as the resolver (optimistic concurrency control) and log servers (crash recovery).  
Figure~\ref{fig:fdb_write_utilization} shows this overhead of the cache in the form of a higher CPU utilization (3x), disk utilization (more than 4x), and network traffic (almost 5x).
These do not slow down the performance of reads because our design populates the cache asynchronously.
With FDB, its read path is separate from its write path.  And, our design and implementation of a sub-query cache maintains this separation.

With $\widehat W$, the disks used by FDB's transaction nodes (log servers) exhibit a high utilization without the cache, 80-90\% with $C^-Q^-$ in Figure~\ref{fig:fdb_write_utilization}.  Our application inserts new data and the sub-queries reference this data, observing cache misses that cause the asynchronous CP threads to populate the cache with new entries.  These writes increase the disk utilization to 94-96\% with $C^+Q^+$ in the same figure.
We tried to reduce the disk utilization by increasing the number of transaction nodes 2x and 3x.
The disk utilization remains unchanged because of FDB's design that requires log records and their meta-data to be written to all log servers, see Section 2.4.3 of~\cite{fdb_sigmod_2021}.
Surprisingly, this higher disk utilization does not degrade the response of writes with $C^+Q^+$ as detailed in Section~\ref{sec:write_fine}.

% The space overhead of the cache is negligible.  We quantified this overhead by comparing the size of the production database with the test database.
% The test database is larger because it contains the key-value pairs corresponding to the cached entries.
% The database size reported by FDB (total size of key-value pairs) is different than the size\footnote{Both are in the order of tens of Terabytes.} of the FDB files occupying a disk, resulting in an overhead of 3.8\% and 2.4\%, respectively.

\subsection{Fine-Grained Analysis of Graph Queries}\label{sec:read_fine}

%https://docs.google.com/spreadsheets/d/1NTmC1h0T1_D6BXtSqhWFpGVlS48Gta6sIglGwta2O5c/edit?gid=634490578#gid=634490578
We selected the top 27 query templates where the traffic percentage is greater than or equal to 1\%. These queries constitute approximately 90\% of the total read traffic\footnote{Note that these queries include those that do not use query re-writing or the cache, e.g., Q1.  If those queries that do not use the cache are subtracted then approximately 68\% of read traffic uses one-hop sub-query templates.}. 
Column 2 of Table~\ref{tbl:query_template_latency} shows the breakdown for the percentage of traffic attributed to each query.
Not all queries can be re-written, see Column 3 of Table~\ref{tbl:query_template_latency}. 
Column 4 shows the one-hop sub-query templates referenced by each query.
A one-hop sub-query template may be referenced multiple times by a query.
This is shown in parenthesis next to the one-hop sub-query template.
%The number in parenthesis is the number of one-hop sub-queries referenced by a query.
The remaining columns show the factor of improvement in latency observed with original query with query rewrite $C^-Q^+$, cache $C^+Q^-$, and both $C^+Q^+$.
We show this with both the 95$^{th}$ and 99$^{th}$ latency.
We consider a difference less than 15\% as experimental noise.
Thus, a factor of improvement from 0.85 to 1.15 is considered insignificant and ignored.
%experimental noise.  

These results highlight the following lessons:
\begin{enumerate}
    \item Query re-writing enhances the latency of a few queries.  See the column $C^{-}Q^{-}$.% and $Q6$.
    \item The cache enhances both the 95$^{th}$ and 99$^{th}$ percentile latency for almost all queries.  See the column $C^{+}Q^{-}$.
    \item The cache in combination with query re-writing provides the highest benefit for almost all queries with a few exceptions ($Q20$ and $Q21$).  See the column $C^{+}Q^{+}$.
%    \item The cache provides the highest factor of improvement with the 95$^{th}$ percentile latency followed with the 99$^{th}$ percentile latency.  With the 95$^{th}$ percentile latency, the improvements observed with some queries are more than 10x with a high system load dominated by either reads or writes, $\widehat R$ and $\widehat W$ workloads.
%    \item Query re-writing enhances latency for a few queries, e.g., Q6 of the column $C^{-}Q^{+}$.
    \item The cache improves the performance of both the original and re-written queries.  This is true with all three system loads.  
\end{enumerate}







\begin{table}[!ht]
    \centering
    \begin{tabular}{|c|c||c|c||c|c|}




        \hline
        \multirow{2}{*}{Workload} & Experiment & \multicolumn{2}{c||}{{\textbf{95$^{th}$}}} & \multicolumn{2}{|c|}{{\textbf{99$^{th}$}}} \\
    \cline{3-6}
        & Day & C$^+$Q$^-$ & C$^+$Q$^+$ & C$^+$Q$^-$ & C$^+$Q$^+$ \\ \hline \hline


\multirow{4}{*}{%\rotatebox[origin=c]{90}{$\widehat R$}
$\widehat R$} & Day 1 & 10.33 & 10.33 & 1.54 & 1.52 \\
           & Day 2 & 9.09 & 9.09 & 1.75 & 1.76 \\
           & Day 3 & 12.71 & 12.71 & 1.76 & 1.74 \\
           & Day 4 & 13.00 & 11.38 & 1.73 & 1.69 \\
\hline 

\multirow{4}{*}{%\rotatebox[origin=c]{90}{$\widehat W$}
$\widehat W$} & Day 1 & 10.33 & 10.33 & 1.54 & 1.52 \\
           & Day 2 & 9.43 & 9.43 & 1.46 & 1.49 \\
           & Day 3 & 6.43 & 4.50 & 1.35 & 2.15 \\
           & Day 4 & 8.83 & 8.83 & 1.37 & 1.41 \\
\hline 


\multirow{4}{*}{%\rotatebox[origin=c]{90}{$\widecheck R$}
$\widecheck R$} & Day 1 & 1.86 & 1.63 & 1.90 & 1.84 \\
           & Day 2 & 1.50 & 1.50 & 1.79 & 1.93 \\
           & Day 3 & 1.60 & 1.60 & 1.72 & 2.04 \\
           & Day 4 & 2.00 & 2.00 & 1.73 & 1.79 \\
\hline    

%\hline
    \end{tabular}
    \caption{Factor of improvement in 95$^{th}$ and 99$^{th}$ latency of Q2 with 3 different workloads.}
    \label{tbl:707ceecd}
\end{table}

Table~\ref{tbl:707ceecd} shows the factor of improvement observed with $Q_2$ on different days with the alternative workloads.
$Q_2$ constitutes 4.2\%-5.2\% of the system load. 
The cache improves its 95$^{th}$ percentile latency by almost 10x with $\widehat R$ and $\widehat W$.
The factor of improvement with $\widecheck R$ is also significant.
The same is observed with the 99$^{th}$ percentile latency.
These observations hold true across all 4 evaluation days.
A pleasant surprise is that the cache provides a benefit with the write heavy $\widehat W$ workload.
The next section describes this observation in greater detail.

\begin{table}[!ht]
    \centering
    \begin{tabular}{|c|cc|cc|cc|}
    \hline
    \multirow{2}{*}{}    & \multicolumn{2}{c|}{August 25} & \multicolumn{2}{c|}{August 26} & \multicolumn{2}{c|}{August 27} \\
    \cline{2-7}
        & Original & Rewrite & Original & Rewrite & Original & Rewrite  \\
    \hline
    \hline
         $\widehat R$&  4.54 & 1.43 & 2.60 & 2.20 & 2.75 & 2.60 \\ \hline
         $\widehat W$&  7.83 & 7.50 & 7.00 & 11.75 & 7.60 & 4.33 \\ \hline
         $\widecheck R$&  5.09 & 6.22 & 4.43 & 4.54 & 6.11 & 6.11\\ \hline
    \end{tabular}
    %\caption{Factor of improvement observed by indirect beneficiaries of the cache, 14.2\% of workload, cache enabled, 95$^{th}$\%.}
    \caption{Factor of improvement observed by an indirect beneficiary of the cache, Q1's 95$^{th}$\% latency.}
    \label{tbl:restofqueries95}
\end{table}

\begin{table}[!ht]
    \centering
    \begin{tabular}{|c|cc|cc|cc|}
    \hline
    \multirow{2}{*}{}    & \multicolumn{2}{c|}{August 25} & \multicolumn{2}{c|}{August 26} & \multicolumn{2}{c|}{August 27} \\
    \cline{2-7}
        & Original & Rewrite & Original & Rewrite & Original & Rewrite \\
    \hline
    \hline

         $\widehat R$& 1.68 & 1.77 & 1.50 & 1.48 & 1.44 & 1.52 \\ \hline
         $\widehat W$& 1.59 & 1.54 & 1.50 & 1.59 & 1.47 & 1.73\\ \hline
        $\widecheck R$& 1.72 & 1.72 & 1.70 & 1.68 & 1.74 & 1.82 \\ \hline
    \end{tabular}
    %\caption{Factor of improvement observed by indirect beneficiaries of the cache, 14.2\% of workload, cache enabled, 99$^{th}$\%.}
    \caption{Factor of improvement observed by an indirect beneficiary of the cache, Q1's 99$^{th}$\% latency.}
    \label{tbl:restofqueries99}
\end{table}

Approximately 14\% of the read workload consists of an aggregate query Q1 that does not have a re-write.
It does not consist of a sub-query and does not use the cache.
Still, Q1 benefits greatly from the use of the cache, see Tables~\ref{tbl:restofqueries95} and~\ref{tbl:restofqueries99}. 
Its 95$^{th}$ percentile with the original queries improves several folds, at times more than 11x.  See Table~\ref{tbl:restofqueries95}.  Its 99$^{th}$ percentile improves by at least 1.4x, see Table~\ref{tbl:restofqueries99}.
These improvements are observed with both the original query and its re-writing.
The explaination for these significant improvements is as follows.
The cache reduces the overhead of query processing, reducing the load on Graph-QPs and FDB instance. 
These freed resources expedite the processing of queries that do not use the cache.
%Its improvement is not as dramatic as the 95$^{th}$ percentile.


\subsection{Fine-Grained Analysis of Writes}
\label{sec:write_fine}

Our application consists of three types of writes: (1) Update or insert (Upsert) a sub-graph consisting of several vertices and edges between them, (2) Update last-seen edges, and (3) Delete edges. Vertices are never removed. Each write is more correctly a read-write request, where it retrieves the graph data and subsequently may update the graph by evaluating a predicate. For example, Type 1 adds a vertex if one does not exist.
Otherwise, it may update some existing properties of the vertex. A write request may not apply its change to the graph if its conditions 
%for introducing new changes are all 
are not satisfied. For example, 
%a write of Type 1 is a no-op operation 
a Type 1 write is a no-op if all its specified vertices and edges already exist and their properties are identical with those specified by the write. Table~\ref{tbl:write_breakdown} breaks down the writes with the different workloads.
It shows the average number of changes (vertices and edges) per write and the average changes per write that impact at least one cache entry.
With a write heavy workload $\widehat W$, more than 25\% of the changes to the graph have no impact on a cache entry, compare 2.08 with 1.52 in Table~\ref{tbl:write_breakdown}.
This is because certain changes do not impact the result of a one-hop sub-query template, e.g., modifying the value of a property that is not referenced by a sub-query template.
%as discussed in Section~\ref{sec:writes}
%Many writes do not change the graph.
Hence, while the percentage of writes is high in Table~\ref{tbl:workload_periods} (34\%), the actual writes that incur the overhead of invalidating impacted cache entries is lower.



\begin{table}[!ht]
    \centering
    \begin{tabular}{|l|c|c|}
        \hline
        Period & Avg. changes & Average changes per write impacting \\
         & per write & at least one cache entry \\ \hline \hline
        $\widehat R$ & 1.31 & 0.98 \\ \hline
        $\widehat W$ & 2.08 & 1.52 \\ \hline
        $\widecheck R$ & 2.99 & 2.23 \\ \hline
    \end{tabular}
    \caption{Average changes per write in different periods.}
    \label{tbl:write_breakdown}
\end{table}

A write transaction impacts a few cache entries most of the time.
Table~\ref{tbl:write_impacted_cache_keys} shows the number of impacted cache keys by each type of write. The numbers shown are from a 25-minute measurement of $\widehat W$, thus sufficient to get the insights without loss of generality.
At the 50th percentile, the number of impacts keys is zero with all three types of writes.  \emph{Update Last-Seen} impacts none of the six sub-query templates.  Upsert impacts the highest number of keys when considering the 95$^{th}$ and 99$^{th}$ percentile.
At the 99$^{th}$ percentile, only a few dozens of cache keys are impacted.
At its extreme, a write impacts 2516 cached keys.
This write consists of 3 updates.
One changes the leaf vertex's property value,
impacting all 2516 keys because (1) the vertex property  is a part of two sub-query templates' predicates, namely, SQ3 and SQ4, and (2) this vertex has a large number of edges connected to it.
Even with this large number of impacted cache keys, this batch write transaction completes in 1,156 ms.
Our customer considers this latency reasonable for their real-time decision application.

\begin{table}[!ht]
    \centering
    \begin{tabular}{|l|l|l|l|l|l|}
        \hline
        Write Type & Mean & 50$^{th}$ & 95$^{th}$ & 99$^{th}$ & Max \\ \hline \hline
        Upsert Sub-Graph & 4.72 & 0 & 18 & 28 & 2516 \\ \hline
        Update Last-Seen & 0 & 0 & 0 & 0 & 0 \\ \hline
        Delete Edges & 0.26 & 0 & 4 & 8 & 32 \\ \hline
    \end{tabular}
    \caption{Impacted cached keys per write type.}
    \label{tbl:write_impacted_cache_keys}
\end{table}

Table~\ref{tbl:write_heavy_breakdown} shows the factor of improvement in the 95$^{th}$ and 99$^{th}$ latency observed with the cache for the three types of writes.
The cache improves the performance of writes by reducing the overhead of query processing.
In turn, this reduces the imposed load on the Graph-QPs and FDB instances.  It frees resources to expedite the processing of writes, providing the significant improvements shown in 
Table~\ref{tbl:write_heavy_breakdown}.

\begin{table}[!ht]
    \centering
    \begin{tabular}{|l|c|c|c|}
        \hline
        \multirow{2}{*}{Write Type} & \% of & \multicolumn{2}{|c|}{Latency Improvement} \\
        \cline{3-4}
         & Writes & 95$^{th}$ & 99$^{th}$ \\ \hline \hline
        Upsert Sub-Graph & 44.85\% & 1.48 & 1.28 \\ \hline
        Update Last-Seen & 43.94\% & 2.13 & 1.48 \\ \hline
        Delete Edges & 11.22\% & 2.14 & 1.39 \\ \hline
    \end{tabular}
    \caption{Different types of write with $\widehat W$ and the factor of improvement observed with the cache.}
    \label{tbl:write_heavy_breakdown}
\end{table}

\subsection{Error Rate}
The two major causes of errors are \emph{time-outs} and \emph{write transaction conflicts}. The former is because some queries retrieve and process a large amount of data that exceed the 5-second transaction limit enforced by FDB. The latter is because concurrent write transactions may have read-write conflicts that cause only one to commit while the others abort due to FDB's use of the optimistic concurrency control protocol.
Table~\ref{tbl:error_rate} shows the rate of error for the three workload periods.
By reducing latency, caching and query rewrites minimize the rate of errors.
By enabling only one, the error rate is reduced 1.16-2.8x.
With both enabled, the error rate is reduced significantly, 4.98-6.32x.
See the last column of Table~\ref{tbl:error_rate}.

%These conflicts are reduced with either query-rewriting or caching as results of reducing latency. Both caching and query-rewriting are effective ways to reduce latency. We observed improvements in error rate when enabling them one by one (1.16-2.8x). Combining both results in significant reductions in error rate in all the three chosen periods (4.98-6.32x).

\begin{table}[!ht]
    \centering
    \begin{tabular}{|l|l|l|l|l|l|l|l|}
        \hline
        \multirow{2}{*}{\textbf{Period}} & \multicolumn{4}{|c|}{\textbf{Error Rate}} & \multicolumn{3}{|c|}{\textbf{Improvement}} \\ \cline{2-8}
         & {\scriptsize C$^-$Q$^-$} & {\scriptsize C$^+$Q$^-$} & {\scriptsize C$^-$Q$^+$} & {\scriptsize C$^+$Q$^+$} & {\scriptsize C$^+$Q$^-$} & {\scriptsize C$^-$Q$^+$} & {\scriptsize C$^+$Q$^+$} \\ \hline\hline

        $\widehat R$ & 0.39\% & 0.25\% & 0.20\% & 0.08\% & 1.45 & 1.97 & 4.65 \\ \hline
        $\widehat W$ & 0.39\% & 0.34\% & 0.15\% & 0.08\% & 1.16 & 2.70 & 4.98 \\ \hline
        $\widecheck R$ & 0.56\% & 0.45\% & 0.20\% & 0.09\% & 1.24 & 2.80 & 6.32 \\ \hline
    \end{tabular}
    \caption{Error rates of alternative configurations and factor of improvement using the cache and query rewrite.}
    \label{tbl:error_rate}
\end{table}

\color{blue}
%\subsection{Resource Utilization}



%Fig~\ref{fig:resource_utilization} shows the total resource utilization of Graph-QP nodes, FDB storage and transaction nodes for the 4 configurations with $\widehat R$. With either enabling or disabling query rewriting, enabling cache reduces CPU consumption on graph processors significantly, see Fig~\ref{fig:gp_utilization}. On each graph processor, FDB client uses one thread to handle network IO to FDB cluster. With cache, total CPU consumption on FDB network thread is half as it is without cache.

%Snapshot reads are served directly from FDB storage nodes. With cache, FDB storage nodes have lower CPU utilization, disk utilization. Network sent rate is reduced significantly by 4x, see Fig~\ref{fig:fdb_storage_utilization}.

%Cache introduces more write coming from both read and write path. On reads, background cache population populates cache entries. On writes, besides graph changes, impacted cache keys are deleted (with invalidation technique). FDB transaction nodes, hence, shows remarkably higher CPU, disk and network utilization, see Fig~\ref{fig:fdb_transaction_utilization}. 

}

==> evalNewoneQueryTable.tex <==

\begin{table}[!ht]
    \centering
    \begin{tabular}{|c|c||c|c||c|c|}




        \hline
        \multirow{2}{*}{Workload} & Experiment & \multicolumn{2}{c||}{{95$^{th}$ Latency}} & \multicolumn{2}{|c|}{{99$^{th}$ Latency}} \\
    \cline{3-6}
        & Day & C$^+$Q$^-$ & C$^+$Q$^+$ & C$^+$Q$^-$ & C$^+$Q$^+$ \\ \hline \hline


\multirow{4}{*}{%\rotatebox[origin=c]{90}{$\widehat R$}
$\widehat R$} & Day 1 & 10.33 & 10.33 & 1.54 & 1.52 \\
           & Day 2 & 9.09 & 9.09 & 1.75 & 1.76 \\
           & Day 3 & 12.71 & 12.71 & 1.76 & 1.74 \\
           & Day 4 & 13.00 & 11.38 & 1.73 & 1.69 \\
\hline 

\multirow{4}{*}{%\rotatebox[origin=c]{90}{$\widehat W$}
$\widehat W$} & Day 1 & 10.33 & 10.33 & 1.54 & 1.52 \\
           & Day 2 & 9.43 & 9.43 & 1.46 & 1.49 \\
           & Day 3 & 6.43 & 4.50 & 1.35 & 2.15 \\
           & Day 4 & 8.83 & 8.83 & 1.37 & 1.41 \\
\hline 


\multirow{4}{*}{%\rotatebox[origin=c]{90}{$\widecheck R$}
$\widecheck R$} & Day 1 & 1.86 & 1.63 & 1.90 & 1.84 \\
           & Day 2 & 1.50 & 1.50 & 1.79 & 1.93 \\
           & Day 3 & 1.60 & 1.60 & 1.72 & 2.04 \\
           & Day 4 & 2.00 & 2.00 & 1.73 & 1.79 \\
\hline    

%\hline
    \end{tabular}
    \caption{Factor of improvement in 95$^{th}$ and 99$^{th}$ latency of a graph query with 3 different workloads.}
    \label{t

==> figAllUtil.tex <==
\begin{figure*}[htbp]  % htbp defines position as here, top, bottom, page

    % Group 1 (Top: 2 Charts)
    \begin{subfigure}{\linewidth}
        \centering
        \begin{subfigure}{0.45\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/Graph-QP Core.pdf}
        \end{subfigure}
        \hspace{0.05\linewidth}
        \begin{subfigure}{0.45\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/Graph-QP FDB Network Thread.pdf}
        \end{subfigure}
        \caption{Graph processors}
        \label{fig:gp_utilization}
    \end{subfigure}

    \vspace{1em}  % Space between groups

    % Group 2 (Middle: 3 Charts)
    \begin{subfigure}{\linewidth}
        \centering
        \begin{subfigure}{0.3\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/FDB Storage CPU.pdf}
        \end{subfigure}
        \hspace{0.03\linewidth}
        \begin{subfigure}{0.3\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/FDB Storage Disk Busy.pdf}
        \end{subfigure}
        \hspace{0.03\linewidth}
        \begin{subfigure}{0.3\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/FDB Storage Network Sent.pdf}
        \end{subfigure}
        \caption{FDB storage nodes}
        \label{fig:fdb_storage_utilization}
    \end{subfigure}

    \vspace{1em}  % Space between groups

    % Group 3 (Bottom: 3 Charts)
    \begin{subfigure}{\linewidth}
        \centering
        \begin{subfigure}{0.3\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/FDB Transaction CPU.pdf}
        \end{subfigure}
        \hspace{0.03\linewidth}
        \begin{subfigure}{0.3\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/FDB Transaction Disk Busy.pdf}
        \end{subfigure}
        \hspace{0.03\linewidth}
        \begin{subfigure}{0.3\linewidth}
            \centering
            \includegraphics[width=\linewidth]{figs/FDB Transaction Network Sent.pdf}
        \end{subfigure}
        \caption{FDB transaction nodes}
        \label{fig:fdb_thread_utilization}
    \end{subfigure}

    \caption{Resource utilization of graph processors and FDB storage/transaction nodes}
    \label{fig:resource_utilization}
\end{figure*}

==> graphQPutil.tex <==
% \begin{figure}[htbp]  % htbp defines position as here, top, bottom, page
%    \centering
%     \begin{subfigure}{0.45\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/Graph-QP Core.pdf}
%     %\caption{Graph-QP CPU Utilization}
%     %\label{fig:graphqp_util}
%     \end{subfigure}

%     %\hspace{0.05\linewidth}
%     \begin{subfigure}{0.45\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/Graph-QP FDB Network Thread.pdf}
%     %\caption{FDB Client Network Thread}
%     %\label{fig:thread_utilization}
%     \end{subfigure}

%     \caption{Graph-QP CPU Utilization with $\widehat R$.}
%     \label{fig:graphQPutil}
% \end{figure}

\begin{figure}[htbp]
    \centering
    % First chart (on the left)
    \begin{subfigure}{0.49\linewidth}  % Use 0.45\linewidth to fit in a single column
        \centering
        \includegraphics[width=\linewidth]{figs/Graph-QP Core.pdf}  % Path to the first PDF
        \caption{Graph-QP CPU Utilization}\label{fig:graph-qp-util}
    \end{subfigure}
    % \hspace{0.05\linewidth}  % Space between the two charts
    % Second chart (on the right)
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/Graph-QP FDB Network Thread.pdf}  % Path to the second PDF
        \caption{FDB Client Network Thread}\label{fig:fdb-thread-util}
    \end{subfigure}

    \caption{Graph-QP CPU Utilization with $\widehat R$.}
    \label{fig:graphQPutil}
\end{figure}

==> queryRewriting.tex <==
\subsection{Query Rewriting}\label{sec:rewrite}
%The cache provides little to no benefit for certain query templates.
%These include (1) queries that retrieve a large amount of data without performing a one-hop traversal, and (2) queries with significant Graph-QP processing time.
%We identified two primary causes for this: (1) the query has additional steps that do not reference the cached sub-queries and retrieve a large amount of data, and (2) the Graph-QP processing time dominates the query execution time.
Certain queries (1) retrieve a large amount of data, and/or (2) incur significant Graph-QP processing time.
The former may perform one or more one-hop sub-query traversals independent of retrieving a large amount of data. 
An example of the latter is merging two sets without sorting.
We apply query re-writing rules to optimize query processing.
%before  query is forwarded to the testing deployment cluster.
%To address inefficient read queries before they are forwarded to the testing deployment cluster, we applied query re-writing strategies to optimize their execution. 
%For our workload, we used the following two optimization rules applicable to multiple query templates:
%Importantly, these rules do not affect the sub-query templates, as both the original and re-written queries utilize identical sub-query templates.
These rules are:
\begin{enumerate}
    \item %Do not retrieve user defined properties with unique values associated with vertices when vertex ids can be used in their stead. An example is given a listing with user defined listing id A, find all watch-lists that have it, and for each watch-list, retrieve all other listings that are different than A. 
    Filter using built-in unique vertex ids instead of user-defined properties with unique values.  Given a vertex id, fetching its property value requires one network round-trip.  The available unique vertex ids eliminates this overhead.
    To illustrate, consider a user defined listing id A with a query to compute all watch-lists that have A and, for each watch-list, retrieve all other listings that are different than A.  
    In this case, JanusGraph-generated vertex ids are sufficient to filter listings that are different than the original listing A.
    This eliminates one round-trip to fetch the value of their user defined properties with unique values.
    %In this case, only using JanusGraph-generated vertex ids is sufficient to filter listings that are different than the original listing A, instead of using user-defined unique ids that requires one more round-trip to fetch their user defined unique values.
    \item Sort before merge. This applies to queries that compute the intersection of two sets consisting of $m$ and $n$ elements. Without sorting, the complexity of computing intersection is $O(m \times n)$. With sorting, the complexity is reduced to $O(M \times log~M)$ where $M=max(m,n)$.
\end{enumerate}
These are applied to a query prior to forwarding it to the test system.
Their application to those queries that reference one-hop sub-queries has no impact on their sub-queries.
Thus, both the original and re-written queries utilize identical sub-query templates and instances.


==> subqueryCache.tex <==

A cache entry is a key-value pair that corresponds to the result of a one-hop sub-query instance.
The key identifies a unique one-hop sub-query instance.
Its value is the output of the one-hop sub-query instance, a list of leaf vertex ids.
We construct the key using (a) the input vertex id, 
%(b) the vertex property names and values referenced by the predicates (if any), 
(b) the direction of a referenced edge, 
(c) the edge property names and values referenced by a predicate, (d) the label used to filter the edge, 
(e) the label used to filter the leaf vertices,
and 
(f) the property names and values referenced by a predicate applied to the leaf vertices.
We maintain a list of all predicates referenced by a sub-query. 
Writes use this list to identify cached keys that should either be invalidated or refilled.

   

\subsection{gR-Txs}

When processing a gR-Tx, the system identifies its list of one-hop sub-query instances and the sequence in which they should be processed.
For a sub-query instance and its root vertex id, it constructs the key of its cached entry.
It looks up the key in the cache.
If the cache produces a value, the query processor (e.g., JanusGraph) has observed a cache hit.
It deserializes the value to obtain a list of leaf vertices.
It uses each resulting vertex id as the root vertex of the next sub-query.
%and enumerates the set of leaf vertices that constitute the root vertex to process the next sub-query.
With a cache miss, the query processor executes the sub-query instance.
%It inserts the sub-query instance and the root vertex id into a queue that is processed by background threads.
It obtains the set of leaf vertex ids produced by this sub-query instance to process the next sub-query instance.
It may populate the cache with the result of a sub-query either synchronously or asynchronously.
It repeats this process until it exhausts all the sub-query instances that constitute the gR-Tx.
It processes the final set of vertices using the final clause of the gR-Tx.
At this point, it has completed processing the gR-Tx and produces the final result set as the output.


%We realize this by populating the cache asynchronously using the CP threads.

We assume vertex ids used to construct the cache keys and their values are immutable. 
In addition, we assume the label of a vertex or an edge is immutable.

%Immutable vertex ids used to construct the cache key and the cached values.
%A cached value consists of a list of vertex ids.
%One or more properties of a vertex may be immutable.
%For example, with JanusGraph, the Label property of a vertex is immutable.

\input{writes}


==> terminology.tex <==


We assume a directed property graph database consisting of vertices (also known as nodes), directed edges, labels, and properties.
Typically, vertices represent entities.
Edges represent connections between vertices and are directed, either going out or into a vertex.
Properties are information added to the vertices and edges.
They are in the form of (attribute, value) pairs.
Vertices and edges may have labels.
Labels identify and group similar types of vertices or edges.



%A traversal query is a sequence of operations that describe how to traverse the graph from one vertex or edge to another.
%edges to identify relevant to retrieve relevant vertices and edges. 
Figure~\ref{fig:sub_query_template_example} presents a compelling example that inspired the development of our caching solution. A watch-list of a user may have multiple listings.
%where each listing may be either active or inactive. 
We model watch-lists and listings as vertices. If a listing is included in a watch-list, there is an edge labeled ``includes'' from the watch-list to the listing. Each listing has a property named ``Status'' with a binary value, either 0 or 1, denoting whether it is available or expired. Moreover, to track a user's behavior, if a listing is excluded from a watch-list, we maintain the edge from the watch-list to the listing and set its ``IsActive'' property value to \texttt{false}. 

A Gremlin traversal query consists of a sequence of operations that describe how to traverse edges of a graph.
An operation may apply a predicate to labels and properties of the vertices and edges.
We assume an operation starts by identifying a root vertex.
It may use predicates to identify its relevant incoming or outgoing edges, pruning the resulting leaf vertices by applying one or more predicates to their labels and properties. 
%They may reference labels and properties of the edges and prune down the resulting vertices by applying a predicate to their labels and properties.
The result is a list of qualifying leaf vertex ids. 
%A traversal query may identify a root vertex by applying a predicate to one or more properties and labels of the vertices.  From this vertex, it may identify its relevant edges, either incoming or outgoing, by examining the property value and label of its edges. This produces a set of leaf vertex ids.
The next operation in the query may use each of these vertex ids as a root vertex and repeat the traversal.
%For each qualifying leaf vertex id, the query may repeat the process of 
%applying a predicate to its property values and those of its edges, producing a new set of leaf vertex ids.   
%The query may navigates the edges of each qualifying vertex id by examining their property value to identify other vertex ids.
This may repeat multiple times until all operations that constitute the query are processed.
The query may use set operators such as union to combine the set of vertices.  
And, with the final set of vertices, it may enumerate a specific property value or apply aggregate functions such as count and group-by~\cite{marko2015}.
The query's final output may be a list of vertices, edges, properties, or any other data extracted from the graph based on the defined operations.

In our example, 
%In Figure~\ref{fig:sub_query_template_example}, 
a watch-list ``BF To-Buys'' consists of 50 listings where 30 edges are active.
A user may be interested in only active listings that have not expired, i.e., Status=0.
%The user might only interested in active listings and wants to retrieve all active listings in his on their watch-list. 
Figure~\ref{fig:sub_query_template_example} shows the corresponding Gremlin query.



We identify the one-hop sub-query instances that constitute a query and cache their resulting vertex ids.
When processing a gR-Tx, we identify its sub-queries and look up their results in the cache first.  We process a sub-query only if its result is not found in the cache.  Otherwise, we proceed to process the obtained vertex ids from the cache to continue the next step of the gR-Tx.



\begin{definition}
A {\em one-hop sub-query instance} consumes one root vertex id to output a set of leaf vertex ids.
It may navigate either the incoming or outgoing edges of the root vertex by applying a predicate to either the property values of its edges, their labels, or both.
It may qualify a leaf vertex by applying one or more boolean predicates to its property values, labels, or both.
The leaf vertex ids are the output of a one-hop sub-query.
Their number is the cardinality of the sub-query.
It may range from zero (output is the empty set) to a large value (output of a super-node with many qualifying edges and leaf vertices). 


%A {\em sub-query} inputs one vertex id to output a set of vertex ids. It computes its output by examining the value of properties associated with its input vertex and its edges. The number of vertex ids in the output is the cardinality of the sub-query. It may be zero (output is the empty set) to a large value (output of a super vertex with many qualifying edges). 
\end{definition}

\begin{definition}
A {\em one-hop sub-query template} identifies the structure of a sub-query instance that is cached.
In addition to values, it may use wildcard characters such as '?' or '$\star$'.
%as the value used by an instance.
A wild card qualifies all possible values as a match.
% for a predicate.
It is possible for a sub-query template to use a value instead of a wildcard.
In this case, only sub-query instances with the matching value are cached.
\end{definition}
A one-hop sub-query instance must match a one-hop sub-query template in order for it to be cached.
Otherwise, it is not cached and writes will not invalidate or refill its cache entry.
The use of a value in a one-hop sub-query template is justified when a large percentage of gR-Txs use the value.
See Section~\ref{sec:discuss} for details.

%{\bf Show with an example.}
%{\color{blue}



%\subsection{A Motivating Example}

With the example query of Figure~\ref{fig:sub_query_template_example},
%Using FoundationDB (FDB) as its transactional storage manager, JanusGraph stores properties and incoming/outgoing edges of vertices as sorted key-value pairs, see Figure~\ref{fig:sub_query_template_example}.
%With the physical layout of a graph database such as JanusGraph~\cite{}, properties and incoming/outgoing edges of a vertex are stored consecutively as key-value pairs in an ordered key-value store. 
%To retrieve all edges or all properties of a vertex, a getRange request is issued to the storage backend. With our example query, first of all the JanusGraph id of the watch-list vertex is retrieved via index. A getRange request is then used to retrieve all 50 edges. The edges are examined to filter only the ones that are still active and identify the corresponding listing ids (encoded as part of the edge ids). For each listing, a getRange request is issued to retrieve their "Status" property to evaluate ``Status=0''. In the end, only 30 listing are valid and their ids are returned.
a graph query execution engine such as JanusGraph processes the query as follows. 
%JanusGraph processes the query as follows.
First, it retrieves the id of the watch-list vertex using an index.
Subsequently, it issues a range selection predicate to retrieve all 50 edges and their property values, see \textcircled{1} in Figure~\ref{fig:sub_query_template_example}.
It filters those edges that satisfy the predicate ``IsActive=true", identifying the 30 qualifying edges that, in turn, identify listings (encoded as a part of the edge ids).  
For each listing, it issues a second range selection predicate to retrieve its ``Status" property and filter those that satisfy the predicate ``Status=0", see \textcircled{2} in Figure~\ref{fig:sub_query_template_example}.
Only 30 listings satisfy this predicate and their vertex ids are returned to the client. Thus, processing of this query requires two network round-trips plus local processing to filter the qualifying vertices. %Queries with the same template that fetch more data in either \textcircled{1} or \textcircled{2} may require more network round-trips when a batch size for a multi-retrieval optimization is applied.
If there were 300 or more listings, the number of concurrent network invocations and the amount of data transferred is increased significantly.

%Caching sub-query instances is a good fit for this example.
Caching instances of sub-queries works well in this case.
%A sub-query template for caching fits well in this case. 
%The sub-query template
Its template is \newline{\small\texttt{.outE("includes").has("IsActive",?).inV().has("Status",?)}}\newline 
The key for an instance of this template is SQ1:10:IsActive=true\&Status=0 where SQ1 is the template name, 10 is the JanusGraph vertex id of the watch-list with ``name" equal to ``BF To-Buys", and IsActive=true\&Status=0 is the parameters of the template wildcard. The cache value consists of 30 vertex ids serialized into bytes.

Every time the sub-query observes a cache hit, the two network round-trips are reduced to one for a cache lookup, the amount of data retrieved is reduced, and local processing for evaluating the query predicate is eliminated.


%and the cost of de-serializing a value and local processing (for evaluating the query predicate) is eliminated.
%also reduced significantly.
%With a cache miss, the processing with two network round-trips of getRange requests incurs the additional network round-trip of cache lookup.

A gR-Tx template may consist of multiple one-hop sub-query templates.
%A well-chosen sub-query template can also be used in multiple query templates. 
An example gR-Tx is, given a listing id ``L1",
%For example, another query is given a listing id ``L1'', 
retrieve all other listings that are included in at least one common watch-list with ``L1''.
Its Gremlin query template is:
\texttt{g.V().hasLabel ("Listing").has("id", "?").inE("includes").has("IsActive",
true).outV().hasLabel("WatchList").outE("includes").
has("IsActive",?).inV().has("Status",?).valueMap()}.
It consists of two one-hop sub-query templates:
%Its Gremlin expression consists of one-hop sub-queries \texttt{g.V().hasLabel ("Listing").has("id", "ABC").inE("includes").has("IsAct ive", true).outV().hasLabel("WatchList").outE("includes").
%has("IsActive",true).inV().has("Status",0).valueMap()}.
An instantiation of the first one-hop sub-query template produces a set of leaf vertex ids.
Each vertex id instantiates the second one-hop sub-query instance to reference a cache entry.

%For each such vertex id, 
%The second one-hop traversal of the query matches the defined sub-query template and may reference multiple cache entries, where each cache key is associated with each watch-list vertex found at the first-hop traversal.

%}

\begin{definition}
A {\em super-node} is a vertex with many in-coming, out-going, or a combination of in-coming and out-going edges.  
A super-node may either be a root or a leaf vertex of a one-hop sub-query instance.
When a super-node is the root of a one-hop sub-query, it may result in many traversals to compute the result of the sub-query.  However, it may not produce many leaf vertex ids.
When a super-node is a leaf vertex, it means the super-node appears in the result of many one-hop sub-query instances.
Thus, a gRW-Tx that impacts a super-node may either invalidate or refill many cache entries.
\end{definition}

==> writes.tex <==
\subsection{gRW-Txs}\label{sec:writes}
gRW-Txs either invalidate or refill the cache entries impacted by their writes in a transactional manner.
While invalidate deletes the impacted cache entries, 
refill updates them.
%Performing these operations in a transactional manner means the invalidation and refill operations 
They are performed as a part of the transaction that writes the graph database, preserving the consistency of the cache entries with the graph database state.
A write may consist of one or more of these changes:
\begin{enumerate}
    \item add a new edge between two vertices, $V_{i}$ and $V_{j}$, 
    \item delete an edge between two vertices, $V_{i}$ and $V_{j}$, 
    \item add a property value to an edge between two vertices, $V_{i}$ and $V_{j}$,
    \item delete a property from an edge between two vertices, $V_{i}$ and $V_{j}$,
    \item update a property value of an edge between two vertices, $V_{i}$ and $V_{j}$, 
    \item add a new property with a value to Vertex $V_{i}$, 
    \item delete a property and its value from Vertex $V_{i}$, 
    \item update a property value of Vertex $V_{i}$, 
    \item delete a Vertex $V_{i}$,
    \item add a vertex $V_{i}$.
    %\item perform several of the above as one transaction.
\end{enumerate}
While these writes may impact a cache entry, adding a vertex is a write that does not impact the result of a sub-query, i.e., a cache entry.
Hence, it is not considered.
With the first five, the direction of the edge is important for identifying the impacted cache entries.

Refill has two possible definitions when a write produces a new cache entry that did not exist previously.
An example is a write that adds a new property value to $V_i$, causing some sub-queries to produce a vertex list for $V_i$ that did not exist previously.
One definition of refill is to do nothing.
This will require a future query that references the sub-query with $V_i$ to observe a miss and populate the cache.
%, causing a CP to compute the missing cache entry and populate the cache asynchronously.
Another definition is to require the write operation to populate the cache with the missing new entry, enabling the future query to observe a hit.
The former is advantageous when a future query never references the new cache entry.
The latter is advantageous when many future queries reference the new cache entry almost immediately and frequently. 
Its disadvantage is that it slows down the writes by requiring it to populate the cache synchronously. 
This section assumes the second definition of refill.

In order for a write to process sub-queries to identify the impacted cache entries, it may require the vertex property names and values used by the different sub-queries.
The property names may be obtained once at system initialization time by processing the sub-query templates.
The value of these properties for the impacted vertices may be obtained once before the write identifies the impacted sub-queries.
Below, we describe the different graph writes, how they identify the impacted cache entries, and how they refill these entries.

{\em Add a new edge between two vertices, $V_i$ and $V_j$:}
The direction of the edge is important. 
We assume the edge is outgoing from $V_i$ to $V_j$.
The inverse of this is a simple switch of subscript for the following discussion.

The write computes the impacted cache entries by analyzing the individual sub-query templates.
A sub-query template may traverse an incoming edge, an outgoing edge, or both.
%With out assumption of the direction of the new edge, only the sub-query template with the outgoing edge or both are considered.
%It identifies the different sub-query templates with a predicate that references either the outgoing edge or both the outgoing and incoming edges of a root vertex. Consider each in turn.
We discuss them in turn.
With the first two, it evaluates whether $V_i$ as the root of the sub-query template satisfies $V_j$ as a leaf vertex using the properties of the new edge, $V_i$, and $V_j$.
If affirmative then the result of the sub-query instance using $V_i$ as its root has changed.
The write will construct the impacted key for the query template using $V_i$'s vertex id.
Next, it either delete the corresponding cache entry (invalidate) or refill it by adding $V_j$ to its result set.  
With the second scenario, the write examines the sub-query instance using either $V_i$ or $V_j$ as the root, repeating the above with each as the root vertex.


A sub-query template may reference one or more properties of a leaf vertex, e.g., the \texttt{Status} property in our examples.
The value of this property for the leaf vertex is used to construct the key of an impacted cache entry.
The new edge, $V_i$, and $V_j$ must have the properties referenced by the query template.
Otherwise, the write computes no cached key.

To illustrate, consider the sub-query template of Figure~\ref{fig:sub_query_template_example} and assume the edge being added has an ``IsActive" property and its value is true.
%The above description does not consider the direction of an edge and how it is used by a sub-query.
Since the sub-query traverses the outgoing edges of a root vertex, the write will consider only $V_i$ as the root.
Assume $V_i$=10, the yellow vertex, and we are adding the edge from it to a new Listing vertex, say $V_j$=101, with Status=0.
The write instantiates the query template using the properties of this edge and the listing vertex to construct the impacted key SQ1:10:IsActive=true\&Status=0.
Subsequently, the write either deletes this key as a part of its transaction or refreshes it to include $V_j$=101.

%because the sub-query is interested in the outgoing edges of $V_i$.
%To illustrate, consider the following variation of the above sub-query template:
%{\small\begin{verbatim}__.outE(‘Linking’).has(“IsActive”, *).inV().has(“Status”, *)\end{verbatim}}
%The sub-query template considers the outgoing edges of a root vertex.
%$V_j$'s result with this sub-query will not change with a new outgoing edge from $V_i$ to $V_j$.
%Hence, it is not considered as the root of the sub-query.


%The write fetches the value of the properties referenced by the different sub-queries for the two vertices connected by the new edge.
%Each sub-query is a one-hop traversal from a root vertex to leaf vertices.
%The write examines all registered sub-query templates with either $V_i$ or $V_j$ as the root vertex and $V_j$ or $V_i$ as the child vertex.
%This identify the matching sub-queries.
%This may require the use of $V_1$ and $V_2$ property values and those of the new edge.  As an example, 
Consider the same write with a different sub-query template, SQ6:
\newline{\small\texttt{\_\_.bothE("includes").has("IsActive", *).inV().has("Status", *)}}\newline
With $V_i$=10 as the root and the previous description, 
%the write uses the query processor to evaluate whether the new edge's \texttt{includes} label and \texttt{IsActive} status qualifies $V_j$ as a leaf vertex.  If affirmative then, with refill, $V_j$ is added to the cache entry corresponding to the result of the sub-query instance with $V_i$ as its root.
it computes the impacted cached key SQ6:10:IsActive=true\&Status=0.
Invalidate deletes this cache entry while refill updates the entry with $V_j$=101.
%With invalidate and refill, this cache entry is deleted and updated with $V_j$, respectively.
Next, the write repeats this process with $V_j$=101 as the root.
It detects the child vertex, $V_i$=10, is missing the ``Status" property and terminates.
If $V_i$=10 had the ``Status=1" property then the write would have proceeded to construct the impacted key SQ6:101:IsActive=true\&Status=1.
The write would have either deleted this key or refilled it with $V_i$=10.

%However, this time, the write must repeat this process with $V_j$ as the root, identifying its potential cache entry to either be invalidated or refreshed with $V_i$ added as a leaf vertex since the sub-query uses \texttt{bothE}.
%This is repeated with $V_j$ as the root and $V_i$ as the leaf vertex since the sub-query uses \texttt{bothE}.




%The write fetches the property value of a participating vertex once for all sub-queries that reference it.
%(if it does not have it) in order to identify the cached results of the sub-query.  


{\em Delete an existing edge:}
The process of identifying the impacted cache entries and invalidating them is identical to adding a new edge with one difference.
With refill, a leaf vertex, either $V_i$ or $V_j$, may be deleted from the cached result of a sub-query instance.

{\em Add a property value to an edge:}
This is handled in the same manner as adding a new edge.

{\em Delete a property value of an edge:}
This is handled in the same manner as removing an edge.

{\em Update a property value of an edge:}
This is identical to removing an edge with the old property value and adding a new edge with the new property value.
See the respective writes in the aforementioned paragraphs.
%The write processes each to identify
%them in the same manner, identifying 
%all impacted keys.
It eliminates duplicate keys prior to either invalidating or refilling them.

{\em Add a new property with a value to Vertex $V_{i}$:}
%The write produces a new cache key that did not exist previously.  Hence, it does not invalidate cache entries.
%This write may cause some sub-queries to produce a list of vertex ids and associate them with a key that did not exist previously.
%Per our definition of refill, the write must compute these new cache entries.
%Its details are as follows.
The write identifies all sub-query templates that reference the new property.
A sub-query may apply the predicate to either a root vertex or a leaf vertex.
Consider each in turn.
With the former, the write is generating a cache key that did not exist previously.
Hence, there is no cache entry to delete with invalidate.
%Thus, with invalidate, there is no cache entry to delete. 
With our definition of refill, the write uses $V_i$ as the root of the sub-query and compute its leaf vertices, generating a new cache entry that it inserts in the cache.

With a sub-query that references the new property to qualify a leaf vertex, the write identifies those vertices $\{V\}$ that are one hop away from $V_i$.
It uses each vertex $V_j$ in $\{V\}$ as the root of the sub-query and evaluates whether $V_i$ qualifies by instantiating the sub-query.
If affirmative, with invalidate, the cache entry corresponding to the result of the sub-query instance with $V_j$ as its root vertex is deleted. 
With refill, $V_i$ is added to the cache entry for the sub-query instance and $V_j$ as its root vertex. 

% then $V_j$ is added to the set $\{K\}$. Subsequently, it iterates each key $k$ in $\{K\}$.


{\em Delete a property and its value from Vertex $V_{i}$:}
%A write may delete a property of $V_i$ using the \texttt{drop} command of Gremlin.
%Both refill and invalidate delete the impacted keys.
Similar to adding a new property, the write identifies all sub-query templates with a predicate that reference the deleted property. 
It identifies whether the sub-query applies the predicate to a root vertex, a leaf vertex, or both.
With the root vertex, it uses $V_i$ and its old property value to construct the key of the impacted cache entry for the query template.
It deletes this key with both invalidate and refill.

When a sub-query template uses the old property to qualify leaf vertices, an instance of it may no longer have $V_i$ in its result set.
Hence, the write identifies all such sub-query templates.
Next, it identifies those vertices $\{V\}$ that are one hop away from $V_i$.
With each sub-query template,
it uses a vertex $V_j$ in $\{V\}$ as the root of the sub-query and evaluates whether $V_i$ qualifies with its deleted property and old value.
If affirmative, it constructs the key of each sub-query instance with $V_j$ as its root vertex.
It deletes these keys with invalidate.
With refill, it updates the cache entry by removing $V_i$ from the value of the key.


{\em Update a property value of a vertex $V_i$:}
This is equivalent to first deleting the property with its old value and subsequently adding the property with its new value.  See the previous two types of writes.

\begin{comment}
Logically, such an update is equivalent to first deleting the property with its old value and subsequently adding the property with its new value.
However, this may result in many un-necessary cache invalidation and refills when an update does not change the result of a sub-query.  
%Depending on the old and new values of $V_i$ and the predicates used by the different sub-queries, this write may or may not change the result of a sub-query.
To illustrate, consider the following sub-query:
{\small\begin{verbatim}__.outE(‘Linking’).inV().has('age',inside(21,60))\end{verbatim}}
Its range predicate qualifies leaf vertices with \texttt{age} property values greater than 21 and less than 60.
Assume $V_j$ is a qualifying leaf vertex cached as the result of this sub-query with $V_i$ as its root vertex.
An update that changes the \texttt{age} property of $V_j$ from 50 to 51 has no impact on the result of this sub-query.
Our implementation detects such scenarios and does not invalidate or refill a cache entry.
On the other hand, a change of $V_j$'s \texttt{age} property from 50 to 70 impacts the result of the sub-query, requiring its cache entry to either be invalidated or refilled.

The write detects if it impacts the result of a sub-query as follows.
It identifies the sub-query templates that reference the property being updated. 
In our example, it is the \texttt{age} property.
For each sub-query, it identifies whether the result of the predicate referencing the property changes when switching from the old to the new value.
If the result does not change then there is no impact on the cached query results, requiring no invalidation or refill.
In our example, the result of \texttt{has('age', inside(21,60))} is the same with the old \texttt{age} value of 50 and the new value 51.
However, the result of the predicate is different with the old \texttt{age} value of 50 and its new value of 70.
Hence, the cached query result must be either invalidated or refilled.

Once the write detects the result of the predicate has changed, it identifies whether the predicate 
is applied to the root vertex or a leaf vertex of the sub-query.
In our example, it is applied to a leaf vertex.
In this case, the write identifies the set of vertices \{V\} one hop away from $V_i$ using the edge referenced by the sub-query.
The result of each vertex $V_j$ in \{V\} for the sub-query has changed.  
With invalidate, the write constructs the key of the cache entry using $V_j$ and deletes it. 
With refill, it either adds or deletes $V_i$ from the cache entry of $V_j$ when the result of the selection predicate is either true or false, respectively.

If $V_i$ is the root of the sub-query then its cached result is deleted with both invalidate and refill.  

\end{comment}

{\em Delete a vertex $V_i$:}
The write examines all sub-queries.
For each, it evaluates whether $V_i$ satisfies the predicate applied to the root or a leaf vertex.
With the root vertex and an instantiated sub-query template using $V_i$'s properties and edges, the write constructs the key identifying the cache entry.
It deletes this entry with both invalidate and refill.
With immutable vertex ids, the failure to perform this delete does not impact correctness
because a deleted vertex is not reachable to be used by a sub-query.

With the leaf vertex, the write identifies the set of vertices $\{V\}$ that are one hop away from $V_i$.
For each vertex $V_j$ in $\{V\}$, it instantiates a query template using $V_j$'s properties and edges to determine if $V_i$ is reachable, i.e., qualifies.
If this is the case then it constructs the impacted cache entry using the instantiated query template with $V_j$ as its root vertex. 
This key is deleted with invalidate.
With refill, $V_i$ is removed from the value of the key.

%It uses the discussion of delete a property and its value from a vertex to identify the impacted cache entry, either invalidating or refilling these cache entries.
